SWIFT: On-the-Fly Self-Speculative Decoding for LLM Inference Acceleration

Speculative decoding (SD) has emerged as a widely used paradigm to accelerate LLM inference without compromising quality. It works by first employing a compact model to draft multiple tokens efficiently and then using the target LLM to verify them in parallel. While this technique has achieved notable speedups, most existing approaches necessitate either additional parameters or extensive training to construct effective draft models, thereby restricting their applicability across different LLMs and tasks. To address this limitation, we explore a novel plug-and-play SD solution with layer-skipping, which skips intermediate layers of the target LLM as the compact draft model. Our analysis reveals that LLMs exhibit great potential for self-acceleration through layer sparsity and the task-specific nature of this sparsity. Building on these insights, we introduce SWIFT, an on-the-fly self-speculative decoding algorithm that adaptively selects intermediate layers of LLMs to skip during inference. SWIFT does not require auxiliary models or additional training, making it a plug-and-play solution for accelerating LLM inference across diverse input data streams. Our extensive experiments across a wide range of models and downstream tasks demonstrate that SWIFT can achieve over a 1.3x-1.6x speedup while preserving the original distribution of the generated text. We release our code in https://github.com/hemingkx/SWIFT.

==> alg/swift.tex <==
\begin{algorithm}[t]
\small
\caption{\method}
\label{algo:swift}
\begin{algorithmic}[1]
\Require
Target model $\M_q$ with $L$ layers, input sequence $\boldsymbol{x}$, output sequence $y_1, \dots, y_t$, target sequence length $T$, layer skip ratio $r$, Bayesian optimization function $\operatorname{BO}$, random search function $\operatorname{RS}$, input space $\boldsymbol{l}=\binom{L}{rL}$, Bayesian interval $\beta$, context window $\gamma$, optimization step $o$, tolerance step $\epsilon$, the maximum number of optimization steps $N_o$, the maximum number of tolerance steps $N_\epsilon$, maximum draft steps $N_p$;
\State{\textbf{initialize} $n \gets t, o \gets 0, \epsilon \gets 0$}
\While{$n< T$}
\mydarkcolor{\LineComment{Termination condition of the optimization phase}}
\If{$o < N_o$ and $\epsilon < N_\epsilon$}\Comment{Context-based Layer Set Optimization~(\S\ref{sec:contextlayeroptimization})}
\mydarkcolor{\LineComment{Context Accumulation}}
\If{$n < \gamma$}
\State Pass
\mydarkcolor{\LineComment{Layer Set Optimization}}
\Else
\State Suggest potential layer set candidate 
$\boldsymbol{z} \leftarrow \operatorname{BO}(\boldsymbol{l}) \text{ if } o \text{ \% } \beta = 0  \text{ else } \operatorname{RS}(\boldsymbol{l})$
\State Obtain the draft model $\M_p \leftarrow \left\{\M_q^{(i)} \mid z_i=0, i=1,2, \ldots, L\right\}$
\State Set $y^{\prime}_{i} \leftarrow \arg \max_{y} \log P\left(y\mid \boldsymbol{x}, \boldsymbol{y}_{<i}; \boldsymbol{\theta}_{\M_p}\right), 1 \leq i \leq \gamma$
\State Set $\texttt{matchness} \leftarrow \frac{\sum_{i} \mathbb{I}\left(y_{i} = y^{\prime}_{i}\right)}{\gamma}, 1 \le i \le \gamma$ 
\EndIf

\EndIf
\State Set $p_1, \dots, p_K \gets \textsc{Draft}\left(x_{\leq n}, \M_p\right)$ 
\mydarkcolor{\LineComment{Drafting: sample $K$ drafted tokens}}
\State Sample $\widetilde{x}_i \sim p_i, i=1, \dots, K$
\mydarkcolor{\LineComment{Verification: compute $K+1$ distributions in parallel}}
\State Set $q_{i} \gets \M_q\left(x\mid x_{\leq n}, \widetilde{x}_{<i}\right), i=1, \dots, K+1$
\mydarkcolor{\LineComment{Verification: verify each drafted token}}
\For{$i=1:K$}
\If{$\textsc{Verify}\left(\widetilde{x}_i, p_{i}, q_{i}\right)$}
\State Set ${x}_{n+i} \gets\widetilde{x}_i$ and $n \gets n + 1$
\Else
\State ${x}_{n+i} \gets \textsc{Correct}\left(p_{i}, q_{i}\right)$
\State and Exit for loop.
\EndIf
\EndFor
\State If all drafted tokens are accepted, sample next token ${x}_{n+1} \sim q_{K+1}$ and set $n \gets n + 1$.
\EndWhile
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\small
\caption{\method}
\label{alg:swift}
\begin{algorithmic}[1]
\Require
LLM $p(x|\boldsymbol z^*,x_1, ..., x_t)$ where $x_1, ..., x_t$ is the prompt, $\boldsymbol z^*$ is a vector that represents the specific layers to bypass;
target sequence length $T$;
max draft tokens to generate $K$.
% \textcolor{blue}{The $p(x|\vec{0},x_1, ..., x_t)$ denotes original LLM,}
The $p(x|\vec{0},x_1, ..., x_t)$ denotes original LLM,
% We denote the original LLM as $p(x|\vec{0},x_1, ..., x_t)$, 
where $\vec{0}$ is a zero vector, indicating all layers are used in inference.
\State $i \leftarrow t$
\While{$i < T$}
\For{$j \leftarrow i, ..., i + K$} \Comment{Drafting Stage}
    \State $x_{j+1} \leftarrow \argmax{p(x|\boldsymbol z^*,x_1, ..., x_{j})}$    
    \If{need to exit drafting}
        \State Break
    \EndIf
\EndFor
\For{$i \leftarrow i, ..., j$} \Comment{Verification Stage}
    \If{$x_{i+1} \ne \argmax{p(x|\vec{0}, x_1, ..., x_{i})}$}
        \State $x_{i+1} \leftarrow \argmax{p(x|\vec{0}, x_1, ..., x_{i})}$ 
        \State Break
    \EndIf
\EndFor
\State $i \leftarrow i + 1$
\State If all draft tokens are accepted, 
        generate next token $x_{i+1} \leftarrow \argmax{p(x|\vec{0},x_1, ..., x_{i})}$ and $i \leftarrow i+1$
\EndWhile
\State \textbf{return} $x_1, ..., x_T$
\end{algorithmic}
\end{algorithm}
